Steering MoE LLMs via Expert (De)Activation

Mixture-of-Experts (MoE) in Large Language Models (LLMs) routes each token through a subset of specialized Feed-Forward Networks (FFN), known as experts. We present SteerMoE, a framework to steer MoE models by detecting and controlling behavior-associated experts. We detect key experts by comparing how often they activate between paired inputs that demonstrate opposite behaviors (e.g., safe vs. unsafe). By selectively activating or deactivating such experts during inference, we control behaviors like faithfulness and safety without fine-tuning. Across 11 benchmarks and 6 LLMs, our steering raises safety by up to +20% and faithfulness by +27%. Alternatively, unsafe steering drops safety by -41% alone, and -100% when combined with existing jailbreak methods, bypassing all safety guardrails. Overall, SteerMoE offers a lightweight, effective, and widely applicable test-time control, while revealing unique vulnerabilities in MoE LLMs. https://github.com/adobe-research/SteerMoE

==> figures/layers_rag.tex <==
\begin{figure}[h]
\centering
    % left bottom right top
    \includegraphics[width=0.99\textwidth, trim=0 0 0 0, clip]{figures/files/layers_rag.pdf}
    \caption{
    Layer-wise Absolute Risk Difference Values $|\Delta_i^\ell|$. Experts associated with document faithfulness exhibit stronger activation difference signals in the middle layers of the models.
    }
    \label{fig:layers_rag}
\end{figure}

==> figures/moe_arch.tex <==
\begin{figure}[h]
\centering
    % left bottom right top
    \includegraphics[width=0.45\textwidth, trim=0 0 0 80, clip]{figures/files/moe_arch.png}
    \caption{
    MoE Architecture. \citep{Chawla_2025a}
    }
    \label{fig:moe_arch}
\end{figure}

==> tables/baselines_all.tex <==
\begin{wraptable}{r}{0.55\textwidth}
	\setlength\tabcolsep{5pt}
    \scriptsize
    \centering
    \tabcolsep=0.10cm
    \begin{tabular}{llllllll}
\toprule
 & Model & gpt-oss-120b & OLMoE-1B-7B-0125-Instruct & Qwen3-30B-A3B & Mixtral-8x7B-Instruct-v0.1 & gpt-oss-20b & Phi-3.5-MoE-instruct \\
Steering & Dataset &  &  &  &  &  &  \\
\midrule
\multirow[t]{4}{*}{No Steering} & AdvBenchCore & 100\% & 100\% & 98\% & 76\% & 100\% & 100\% \\
 & ArtPrompt & 58\% & 86\% & 96\% & 52\% & 40\% & 40\% \\
 & FFA & 100\% & 92\% & 48\% & 4\% & 92\% & 100\% \\
 & GCG & 100\% & 98\% & 100\% & 72\% & 100\% & 100\% \\
\cline{1-8}
\multirow[t]{4}{*}{Steered Unsafe} & AdvBenchCore & 90\% & 86\% & 78\% & 44\% & 74\% & 76\% \\
 & FFA & 18\% & 64\% & 48\% & 6\% & 14\% & 60\% \\
 & GCG & 92\% & 56\% & 64\% & 28\% & 44\% & 70\% \\
\cline{1-8}
\bottomrule
\end{tabular}
	\caption{Safe response rates on 50 AdvBench examples (lower = stronger attack). Steering MoE is competitive alone and achieves the best results on recent models when combined with other methods.}
	\label{tab:baselines_all}
\end{wraptable}

